Reducing model bias in a deep learning classifier using domain adversarial neural networks in the MINERvA experiment

We present a simulation-based study using deep convolutional neural networks (DCNNs) to identify neutrino interaction vertices in the MINERvA passive targets region, and illustrate the application of domain adversarial neural networks (DANNs) in this context. DANNs are designed to be trained in one domain (simulated data) but tested in a second domain (physics data) and utilize unlabeled data from the second domain so that during training only features which are unable to discriminate between the domains are promoted. MINERvA is a neutrino-nucleus scattering experiment using the NuMI beamline at Fermilab. $A$-dependent cross sections are an important part of the physics program, and these measurements require vertex finding in complicated events. To illustrate the impact of the DANN we used a modified set of simulation in place of physics data during the training of the DANN and then used the label of the modified simulation during the evaluation of the DANN. We find that deep learning based methods offer significant advantages over our prior track-based reconstruction for the task of vertex finding, and that DANNs are able to improve the performance of deep networks by leveraging available unlabeled data and by mitigating network performance degradation rooted in biases in the physics models used for training.

==> sec_danns_subsec_overfit.tex <==
\subsubsection{Overfitting study}
\label{sec:overfitstudy}

To test the overfitting hypothesis, we built scenarios where we forced the model to overfit by using a very small training sample and turning off the dropout layers in our network.
In this case, we observed in, for example Figure \ref{fig:dann_vs_nodann_1ksample_losses}, delayed onset of overfitting when using a DANN, which supports our hypothesis.
%In the first of those Figures, we disable dropout, but in the second we re-enable dropout layers and observe delayed overfitting in both the vanilla and DANN-partner networks, which demonstrates our ability to control the early onset of overfitting, as expected. 
%maybe need to define what 'vanilla' means here?

%%% FIGURE SOURCE: https://minerva-docdb.fnal.gov/cgi-bin/private/ShowDocument?docid=16716
\begin{figure}
   \begin{subfigure}{0.5\textwidth}
         \centering
               \includegraphics[width=0.99\linewidth]{FSI_model_trainFSI_testFSI_DCNN_overfit_rndm} 
                \caption{Loss vs Epoch (no DANN)}
                 \label{fig:DCNN_overfit}
        \end{subfigure}
        \begin{subfigure}{0.5\textwidth}
         \centering 
               \includegraphics[width=0.99\linewidth]{FSI_model_trainFSI_testFSI_DANN_overfit_rndm}  
                \caption{Loss vs epoch (DANN)}
                \label{fig:DANN_overfit}
	\end{subfigure}   
  \caption{Here we study Low Energy beam events with FSI and use a very small training set (1,000 events), with drop-out disabled in an effort to force the networks to over-fit.
  We run 10 trials with DANNs (right) and without (left), using randomly initialized weights for the network each time.
  The vertical solid line shows the mean position of the inflection point in the loss curve, with the heavy (light) dashed lines showing the first (second) standard deviation around that mean.
  We can see the sample with a DANN partner targeting a domain with no FSI begins to over-fit the data later than a sample with no DANN partner (epoch 70 vs epoch 45).}
  \label{fig:dann_vs_nodann_1ksample_losses}
\end{figure}

%% don't need the no-dropout version of this
%\begin{figure}
%  \centering
%  \includegraphics[width=0.65\textheight]{dann_vs_nodann_1ksample_losses_withdropout}
%  \caption{Similar to Figure \ref{fig:dann_vs_nodann_1ksample_losses}, we use a very small training set (1,000 events) and study Low Energy beam events with FSI, but now we re-enable drop-out.
%  We can see again that the sample with a DANN partner targeting a domain with no Final State Interactions begins to over-fit the data later than a sample with no DANN partner.
%  We can also see that re-instating drop-out during training delays the onset of over-fitting, as expected.}
%  \label{fig:dann_vs_nodann_1ksample_losses_withdropout}
%\end{figure}




==> sec_future_work.tex <==

%\minerva simulates pile-up by overlaying information directly from data on top of the simulation.
%We simulate the operation of detector readout electronics, so dead-time induced by activity in the overlay is included.
%Event overlay slightly biases the overall energy in a beam spill to the high side, we estimate it is small and has at most a 2\% effect on physics analysis, which is accounted for where appropriate.
%% don't really need to cite \cite{overlaybias}
%While simulating beam pile-up effects from simultaneous neutrino interactions inside the detector is reasonably straightforward, a proper simulation of the hall particles is very difficult and expensive in terms of development and computer time.
%
%Pile-up is a source of problems for the vertex classifier because the neural network will find vertices in the target region that come from pile-up while the event of interest (defined here by a muon track that was charge and momentum analyzed in the MINOS Near Detector) is elsewhere in the detector. 
%See, for example, Figures \ref{fig:evtdisp_117200_712_462} and \ref{fig:evtdisp_117200_204_295}. 
%%While this is something the neural network is sensitive to, we don't have alternative simulations of the hall and so do not investigate this directly.
%We ameliorated pile-up by including relative hit times in the input image, but some pile-up failures remain at the few percent level.
%Possible solutions include changing the network structure to include information about the reconstructed muon, for example in a wide-and-deep network \cite{DBLP:journals/corr/ChengKHSCAACCIA16}.

%\begin{figure}
%	\begin{subfigure}{0.32\textwidth}
%    	\centering
%		\includegraphics[width=0.97\linewidth]{evtdisp_117200_712_462_x_view}
%  		\caption{X View.}
%  		\label{fig:evtdisp_117200_712_462_x_view}
%	\end{subfigure}
%	\begin{subfigure}{0.32\textwidth}
%    	\centering
%		\includegraphics[width=0.97\linewidth]{evtdisp_117200_712_462_u_view}
%  		\caption{U View.}
%  		\label{fig:evtdisp_117200_712_462_u_view}
%	\end{subfigure}
%	\begin{subfigure}{0.32\textwidth}
%    	\centering
%		\includegraphics[width=0.97\linewidth]{evtdisp_117200_712_462_v_view}
%  		\caption{V View.}
%  		\label{fig:evtdisp_117200_712_462_v_view}
%	\end{subfigure}
%	\caption{Simulation run 117200, subrun 712, gate 462. 
%	The black-lines mark the trajectories of particles created by the simulation.
%	For this event, the ``true'' vertex is in the tracker region, but the vertex classifier returns a positive id for an event in target 1 (from pile-up).}
%	\label{fig:evtdisp_117200_712_462}
%\end{figure}
%
%\begin{figure}
%	\begin{subfigure}{0.32\textwidth}
%    	\centering
%		\includegraphics[width=0.97\linewidth]{evtdisp_117200_204_295_x_view}
%  		\caption{X View.}
%  		\label{fig:evtdisp_117200_204_295_x_view}
%	\end{subfigure}
%	\begin{subfigure}{0.32\textwidth}
%    	\centering
%		\includegraphics[width=0.97\linewidth]{evtdisp_117200_204_295_u_view}
%  		\caption{U View.}
%  		\label{fig:evtdisp_117200_204_295_u_view}
%	\end{subfigure}
%	\begin{subfigure}{0.32\textwidth}
%    	\centering
%		\includegraphics[width=0.97\linewidth]{evtdisp_117200_204_295_v_view}
%  		\caption{V View.}
%  		\label{fig:evtdisp_117200_204_295_v_view}
%	\end{subfigure}
%	\caption{Simulation run 117200, subrun 204, gate 295. 
%	The black-lines mark the trajectories of particles created by the simulation.
%	For this event, the ``true'' vertex is in the tracker region, but the vertex classifier returns a positive id for an event in target 5 (from pile-up).}
%	\label{fig:evtdisp_117200_204_295}
%\end{figure}

%%% Geometry
%
%A possible component of the detector response is the geometry of the simulation or the transformation between the strip measurements and the physical location as well as the target locations. While we would expect this to be something that the neural network is sensitive too, we did not have any simulation available with alternative geometries and so did not investigate the sensitivity of the neural network to improperly understood Geometry.

%%% Other things tried
%
%The detector images have as pixels the scintillator strips in a specific plane. The transformation from pixel strips to physical location is not a linear operation for each view nor is it the same for each view. Importantly, only the active strips can detect the path of particles while the passive material and targets do not produce any measurement. Additionally, the spacing or resolution of the U and V views are less dense than the X view. We investigated padding in U and V to represent this lower information density compared to X and also investigated padding for the passive targets and material to account for the non-linearity in the physical transformation between strips and physical position. None of the padding investigated had any positive effect on the performance of the Neural Network.
%
%In other studies where there were multiple views or images for a given event or time, both a concatenated image before convolution and pooling as well as a processing all images or views through convolution and pooling and concatenating the resulting features before the connected layer were used \cite{}. As reported, we primarily used the topology where the views were separated for the convolution and pooling layers and only combined for the fully connected layers. However, we did investigate concatenating the views before the convolution and pooling layers but did not see any positive effect on the performance of the Neural Network by doing this.










